Exploring Semantic Incrementality with Dynamic Syntax and Vector Space Semantics

One of the fundamental requirements for models of semantic processing in dialogue is incrementality: a model must reflect how people interpret and generate language at least on a word-by-word basis, and handle phenomena such as fragments, incomplete and jointly-produced utterances. We show that the incremental word-by-word parsing process of Dynamic Syntax (DS) can be assigned a compositional distributional semantics, with the composition operator of DS corresponding to the general operation of tensor contraction from multilinear algebra. We provide abstract semantic decorations for the nodes of DS trees, in terms of vectors, tensors, and sums thereof; using the latter to model the underspecified elements crucial to assigning partial representations during incremental processing. As a working example, we give an instantiation of this theory using plausibility tensors of compositional distributional semantics, and show how our framework can incrementally assign a semantic plausibility measure as it parses phrases and sentences.

==> cat-dog-example.tex <==
In this instance of the model, the  space $S$  is a two dimensional space with basis vectors true $\top$ and false $\bot$. Sentences that are highly plausible, such as ``dog chases cat'' will have a vector representation close to the True $\top$ basis, sentences that are highly implausible, such as ``orange chases apple'' have a vector close to the False $\bot$ basis. 

\begin{footnotesize}
\begin{center}
\begin{tabular}{|l|cc|}
\hline
 & $\top$ & $\bot$\\
\hline
dog chases cat & 0.9 & 0.1\\
apple chases orange & 0.1& 0.9 \\
\hline
\end{tabular}
\end{center}
\end{footnotesize}

Following \cite{Clark15}, we assume  the space $W$ is built using dependency relations as context and that $W$'s basis vectors denote properties obtained using the output of a dependency parser, e.g.\ as implemented  in \cite{Curran}. For example, \emph{fluffy} can be a basis  of $W$, where  the value entry for the  \emph{dog} at \emph{fluffy} represents the number of times  adjective \emph{fluffy} modified noun \emph{dog} in the corpus. Similarly, \emph{buy} can be a basis and the value entry of the \emph{apple} on \emph{buy} represents the number of times \emph{apple} occurred as the object of \emph{buy} in the corpus. (Numbers here and throughout are invented for expositional purposes, rather than based on real corpus counts -- see \cite{Clark15}).

\begin{footnotesize}
\begin{center}
\begin{tabular}{|l|cccccc|}
\hline
& 1&2&3&4&5&6\\
 & fluffy & run & fast & tasty & buy & juicy\\
\hline
 dog & 0.8 & 0.8 & 0.7 & 0.1 & 0.5 & 0.0\\
 cat&0.9 & 0.8 & 0.6 & 0.0 & 0.5 & 0.0\\
 apple&0.0 & 0.0 & 0.0 & 0.7 & 0.7 & 0.6\\
 orange&0.0 & 0.0 & 0.0 & 1.0 & 0.9 & 1.0\\
\hline
\end{tabular}
\end{center}
\end{footnotesize}


Intransitive verbs  will have matrix representations in the space $W \otimes S$,  with basis vectors as pairs $\langle \text{b},\top\rangle$ or $\langle \text{b},\bot\rangle$.  A high value for a verb  $v$ on the former means that it is highly plausible that $v$   has the property $\text{b}$, i.e. since they have occurred together to a large extent  in the corpus. A high value at the  latter basis means the opposite: that it is highly implausible that $v$ has property $\text{b}$, since they did not occur much together in the corpus. For example, $T^{sleep}$ will have a high value at $\langle \text{fluffy},\top\rangle$, since it is highly plausible that fluffy things  sleep; and a high entry at  $\langle \text{tasty},\bot\rangle$, since it is highly implausible that tasty things (e.g.\ apples)  sleep. $T^{rot}$ has a different plausibility distribution for fluffy and tasty agents:

\begin{footnotesize}
\begin{center}
\begin{tabular}{|l|cccccccc|}
\hline
& 1&2&3&4&5&6& $\cdots$ & 12\\
 & 
 $\langle \text{fluffy} ,\top\rangle$ & 
 $\langle \text{fluffy} ,\bot\rangle$ & 
 $\langle \text{run} ,\top\rangle$&
 $\langle \text{run},\bot \rangle$&
 $\langle \text{tasty},\top \rangle$ &
 $\langle \text{tasty},\bot \rangle$ & $\cdots$ &
$\langle \text{juicy},\bot \rangle$ \\
\hline
sleep & 0.9 & 0.2 & 0.9 & 0.2 & 0.1 & 0.6 & $\cdots$& 0.0 \\
rot & 0.0 & 1 & 0.0 & 1.0 & 0.6 & 0.4& $\cdots$ & 0.9 \\
\hline
\end{tabular}
\end{center}
\end{footnotesize}

Similarly, a transitive verb such as \emph{chase} will have a tensor representation  $T^{chase}$ in the space $W \otimes S \otimes W$, wherein a basis is either a tuple $\langle \text{b}_1,\top,\text{b}_2\rangle$, e.g.\ $\langle \text{fluffy},\top,\text{fluffy}\rangle$, where a high value indicates high plausibility that fluffy things chase fluffy things; or a tuple    $\langle \text{b}_1,\bot, \text{b}_2\rangle$, e.g.\ $\langle \text{tasty},\bot,\text{juicy}\rangle$, where a high value indicates high implausibility that tasty things (e.g.\ apples) chase juicy things (e.g.\ oranges). 

\begin{footnotesize}
\begin{center}
\begin{tabular}{|l|ccccccc|}
\hline
&1&2&3&4&5&$\cdots$& 72\\
 & $\langle \text{fluffy} ,\top, \text{fluffy}\rangle$ & $\langle \text{fluffy} ,\bot, \text{fluffy}\rangle$ & 
 $\langle \text{fluffy} ,\top, \text{run}\rangle$&
 $\langle \text{fluffy},\top,\text{tasty} \rangle$ &
  $\langle \text{fluffy},\bot, \text{juicy} \rangle$ 
  &$\cdots$&
  $\langle \text{juicy},\bot, \text{juicy} \rangle$ \\ 
\hline
chase & 0.7 & 0.3 & 0.6 & 0.4 & 0.3  & $\cdots$ & 0.0 \\
eat & 0.2 & 0.8 & 0.5 & 0.3 & 0.3  & $\cdots$ & 1.0\\
\hline
\end{tabular}
\end{center}
\end{footnotesize}

The interpretation of a full sentence \emph{dogs chase cats} can be derived by standard tensor contraction given these tensors and vectors, and promises the expected high and low levels of (im)plausibility (given that $\cdots$ represents the parts not shown due to space in the tables above):
%
\begin{footnotesize}
\begin{eqnarray*}
&&T^{dog}_i T^{chase}_{ijk} T^{cat}_k = \\
  &&0.8 \times 0.7 \times 0.9 \top + 0.8 \times 0.3 \times 0.9 \bot +
  0.8 \times 0.6 \times 0.8 \top + 0.8 \times 0.4 \times 0.0 \top + 0.8 \times 0.3 \times 0.0 \bot + \cdots + 0.0 \times 0.0 \times \bot \\
  && = 0.89\top + 0.22\bot +  \cdots\\
&&T^{apple}_i T^{chase}_{ijk} T^{orange}_k = \\
  &&0.0 \times 0.7 \times 0.0 \top + 0.0 \times 0.3 \times 0.0 \time 0.0 \bot +
  0.0 \times 0.6 \times 0.0 \top + 0.0 \times 0.4 \times 1.0 \top + 0.0 \times 0.3 \times 1.0 \bot + \cdots + 0.6 \times 1.0 \times 0.0 \times  \bot \\
  && = 0.00\top + 0.00\bot +  \cdots  \\
\end{eqnarray*}
\end{footnotesize}
%
And, of course, we can now also see how such an interpretation is built incrementally. After parsing only the subject ``dog'', we derive a semantic tree containing the vector for ``dog'' and a tensor for $?W \otimes S$;  tensor contraction of the two gives us a vector in $?S$. The vector \textit{dog} is given in the table for $W$ above. For the tensor of  $?W \otimes S$, we can either use the identity tensor $I$, or sum the tensors of all known elements of the $W \otimes S$ space, that is:


\hspace{-1.5cm}\begin{minipage}{15cm}
\begin{eqnarray*}
&& T^{\oplus} = \\
&& T^{sleep} + T^{rot} + T^{chase \ dog} + T^{chase \ cat} + T^{chase \ apple} + T^{chase \ orange} + T^{eat dog} + T^{eat \ cat} +
T^{eat \ apple}
+
T^{eat \ orange}
\end{eqnarray*}
\end{minipage}

\noindent
This effectively represents the tensor of  all possible verb phrases that might follow ``dog''. The tensors of the intransitive ``sleep'' and ``rot'' are given in the above table; for the transitive verb-object phrases, we must contract each verb tensor with the vector of the corresponding object. For instance, the tensors of  $T^{chase \ dog}$ and $T^{eat \ apple}$  are computed as follows:
%

\hspace{-1.5cm}\begin{minipage}{15cm}\begin{footnotesize}
\begin{eqnarray*}
&&T_{jk}^{chase \ dog} = T_{ijk}^{chase} T_k^{dog}  = \\
&& 0.7 \times 0.8 \langle \text{fluffy}, \top \rangle + 
0.3 \times 0.8 \langle \text{fluffy}, \bot \rangle + 
0.6 \times 0.8 \langle \text{fluffy}, \top \rangle 
+ 0.4 \times 0.1 \langle \text{fluffy}, \top \rangle +
0.3 \times 0.0 \langle \text{fluffy}, \bot \rangle +
 \cdots+
0.0 \times 0.0 \langle \text{juicy}, \bot \rangle
  \\
~
\\
&&T_{jk}^{eat \ apple} = T_{ijk}^{eat} T_k^{apple}   = \\
&& 0.3 \times 1.0 \langle \text{fluffy}, \top \rangle + 0.3 \times 0.8 \langle \text{fluffy}, \bot \rangle +
+ \cdots+
0.6 \times 1.0 \langle \text{juicy}, \bot \rangle
\end{eqnarray*}
\end{footnotesize}
\end{minipage}
%

\noindent
Summing all these tensors and contracting them with the vector of ``dog'' provide us with a vector which has the following entries, the partial semantics for the sentence so far:
%
\begin{footnotesize}
\begin{eqnarray*}
&&T^{dog}_i T_{ij}^{\oplus} = \\
&&0.8 \times 0.7 \times 0.8 \top + 0.8 \times 0.6 \times 0.8 \top + 0.8 \times 0.4 \times 0.1 \top + 0.8 \times 0.3 \times 0.8 \bot + 0.8 \times 0.3 \times 0.0 \bot + \cdots + 1.0 \times 1.0 \times \bot\\
&&= 1.38 \top +  1.52 \bot + \cdots 
\end{eqnarray*}
\end{footnotesize}
%
If the sentence is now continued with ``sleep'', we get a more developed tree whose root node semantics are given by tensor contraction of the tensor of ``sleep''  with the vector of ``dog'', obtaining:
%
\begin{footnotesize}
\begin{eqnarray*}
&& T^{dog}_i T^{sleep}_{ij} = \\
&& 0.8 \times 0.9 \top + 0.8 \times 0.9 \top +  0.1 \times 0.1 \top +  0.8 \times 0.2  \bot +  0.8 \times 0.2  \bot + 0.1  \times 0.6\bot +  \cdots + 0.0 \times 0.0 \bot\\
&&= 1.45 \top + 0.38\bot + \cdots
\end{eqnarray*}
\end{footnotesize}
%
We do not have the full vectors, but based on the entries we have,  we see that plausibility increases when moving from the incomplete  $T^{dog}_i T_{ij}^{\oplus}$  to the complete $T^{dog}_i T^{sleep}_{ij}$. Conceptually speaking, the incomplete phrase will be a dense, high-entropy vector with nearly equal values on $\top$ and $\bot$, whereas the complete phrase (or the more complete phrase), will result in a  sparser vector with more differential values on $\top$ and $\bot$. %Even without access to exact numbers, we see that  $T^{\oplus}$ is much more populated and has many more elements in it than $T^{sleep}$,  thus it will gather much higher values in it   than $T^{sleep}$ has.
Continuation with a less plausible verb, e.g. ``rot'' would result in a reduction in plausibility; and different transitive verb phrases would of course have corresponding different effects. We therefore cautiously view this as an initial step towards a model which can provide the ``error  signal'' feedback assumed in models of expectation during language interpretation \cite{Clark15surfing}. 


==> ex-direct-sum.tex <==
If we take $T^\oplus$ to be the direct sum of all possible intransitive verbs and verb phrases in $?W \otimes S$, then we obtain the following tuple for it:
\begin{eqnarray*}
&&T^\oplus = \\
&&\langle T^{sleep}, T^{rot}, \\
&& T^{chase \ dog}, T^{chase \ cat}, T^{chase \ apple}, T^{chase \ orange},\\
&&T^{eat dog}, T^{eat \ cat}, T^{eat apple}, T^{eat \ orange}\rangle
\end{eqnarray*}

Tensor contraction distributes over direct sum. So contracting the above  with the vector of dog provides us with the following tuple:

\begin{eqnarray*}
&&T^{dog}_i T^{\oplus}_{ij}=\\
&&\langle T^{dog}_i T^{sleep}_{ij}, T^{dog}_i T^{rot}_{ij}, \\
&& T^{dog}_i T^{chase \ dog}_{ij}, T^{dog}_i T^{chase \ cat}_{ij}, T^{dog}_i T^{chase \ apple}_{ij}, T^{dog}_i T^{chase \ orange}_{ij},\\
&&T^{dog}_i T^{eat \ dog}_{ij}, T^{dog}_i T^{eat \ cat}_{ij}, T^{dog}_i T^{eat\ apple}_{ij}, T^{dog}_i T^{eat \ orange}_{ij}\rangle 
\end{eqnarray*}

Each of the entries of this tuple is a vector with coordinates on $\top$ and $\bot$. For now, and in the absence of access to full data (which would involve populating a 72 by 2 entry tensor), we denote these vectors  by symbols, as follows:

\begin{eqnarray*}
&&T^{dog}_i T^{\oplus}_{ij}=\\
&&\langle
a_1\top + b_1 \bot,a_2 \top+b_2\bot, 
a_3\top + b_3\bot, \cdots, a_{10}\top + b_{10} \bot\rangle 
\end{eqnarray*}

The actual vector of $T^{dog}T^{sleep}$ is an element of this tuple, namely:
\[
T^{dog}_i T^{sleep}_{ij} = a_1\top + b_1\bot
\]

There is no direct way  of  deciding which one of the above is more plausible. Bit we can transform the  $T^{dog} T^\oplus$ from a tuple  into a distribution over the whole space (details to be entered) and obtain
\[
T^{dog}_i T^{\oplus}_{ij} = (a_1 + a_2 + \cdots + a_{10}) \top + (b_1 + b_2 + \cdots + b_{10}) \bot
\]
This will result in the same  vector as in the previous case, i.e. when we took $T^{oplus}$ to be the sum of all the possible vectors. 

If we do the Hough-Purver magic and assign probabilities to elements of $T^\oplus$,  then for $T^\oplus$ we obtain:

\begin{eqnarray*}
&&T^{dog}_i T^{\oplus}_{ij}=\\
&&\langle p_1 T^{dog}_i T^{sleep}_{ij}, p_2 T^{dog}_i T^{rot}_{ij}, \\
&& p_3 T^{dog}_i T^{chase \ dog}_{ij}, p_4 T^{dog}_i T^{chase \ cat}_{ij}, p_5 T^{dog}_i T^{chase \ apple}_{ij}, p_6 T^{dog}_i T^{chase \ orange}_{ij},\\
&& p_7 T^{dog}_i T^{eat \ dog}_{ij}, p_8 T^{dog}_i T^{eat \ cat}_{ij}, 
p_9 T^{dog}_i T^{eat \ apple}_{ij}, p_{10} T^{dog}_i T^{eat \ orange}_{ij}\rangle
\end{eqnarray*}

Contracting the above with the vector of dog provides us with 

\begin{eqnarray*}
&&T^{dog}_i T^{\oplus}_{ij}=\\
&&\langle
p_1 (a_1\top + b_1 \bot),
p_2 (a_2 \top+b_2\bot), 
p_3(a_3\top + b_3\bot), \cdots, 
p_{10}(a_{10}\top + b_{10} \bot)
\rangle 
\end{eqnarray*}

Transforming it into a distribution over the whole space will provide us with 
\[
T^{dog}_i T^{\oplus}_{ij} = 
 (p_1 a_1 + p_2 a_2+ \cdots p_{10}a_{10}) \top + 
(p_1 b_1 + p_2b_2 + \cdots + p_{10}b_{10}) \bot
\]
%
This will result in a vector  different from the sum case. The entries of this vectors will have higher values than the vector of $T^{dog} T^{sleep}$ and the previous vector of $T^{dog} T^{\oplus}$. 

Since the distributions have positive entries and add up to 1, the above can be turned into density matrices. For that, we have to work in  $S \otimes S$ as opposed to $S$ and with bases $\top \otimes \top$ and $\bot \otimes \bot$. So the above will/should become as follows:

\[
T^{dog}_i T^{\oplus}_{ij} = 
 (p_1 a_1 + p_2 a_2+ \cdots p_{10}a_{10}) \langle\top, \top\rangle + 
(p_1 b_1 + p_2b_2 + \cdots + p_{10}b_{10}) \langle\bot, \bot\rangle
\]

We can also work with density matrices already at the $T^\oplus$ level, where we have to work in $W \otimes S \otimes W \otimes S$, rather than $W \otimes S$. The doubling of spaces is a standard technique  to go from vectors to  density matrices.  



==> figure2.tex <==
\begin{figure}
\begin{tabular}{cc}
& \vspace*{-0.25cm}\\
%\hspace*{-2cm}
\textit{``mary, \ldots''}
& 
%\hspace*{-2cm}
\textit{``\ldots who \ldots''}

\\

%\hspace*{-2cm}
\begin{tabular}{c}
\dstree{1}{2.5}{
\br{$?Ty(t)$}{
 \lf{$Ty(e),Fo(mary),\diamondsuit$} 
 \lf{$?Ty(\langle e,t\rangle)$}
 }
}
\\
\\
\end{tabular}

&

%\hspace*{-2cm}
\begin{tabular}{cc}
\dstree{1}{2.5}{
\br{$?Ty(t)$}{
 \lf[M]{$Ty(e),Fo(mary)$}
 \lf{$?Ty(\langle e,t\rangle)$}
 }
} 
& \\
& 
\dstree{1}{1.5}{
\br[W]{$?Ty(t)$}{
 \psset{linestyle=dashed}
 %\lf{$\langle \uparrow_* \rangle \langle L^{-1}, 
 \lf{$Ty(e),Fo(mary),\diamondsuit$}
 }
}
\nccurve[ncurv=.6,angleA=270,angleB=160]{->}{M}{W}
\\
\end{tabular}
%\vspace*{-0.5cm}

\\

%\hspace*{-2cm}
\multicolumn{2}{c}{\textit{``\ldots sleeps, \ldots''}}\\ 

\multicolumn{2}{c}{
\hspace*{-1cm}
\begin{tabular}{cc}
\dstree{1}{2.5}{
\br{$?Ty(t)$}{
 \lf[M]{$Ty(e),Fo(mary)$}
 \lf{$?Ty(\langle e,t\rangle),\diamondsuit$}
 }
} 
& \\
& 
\dstree{1}{3.5}{
\br[W]{$Ty(t),Fo(sleep(mary))$}{
 \lf{$Ty(e),Fo(mary)$}
 \lf{$Ty(\langle e,t\rangle),Fo(\lambda x.sleep(x))$}
 }
}
\nccurve[ncurv=.6,angleA=270,angleB=160]{->}{M}{W}
\\
\end{tabular}
}\\
\multicolumn{2}{c}{\textit{``\ldots snores''}}\\

\multicolumn{2}{c}{

\begin{tabular}{cc}
\dstree{1}{3.5}{
\br{$Ty(t),Fo(sleep(mary)\land snore(mary)),\diamondsuit$}{
 \lf[M]{$Ty(e),Fo(mary)$}
 \lf{$Ty(\langle e,t\rangle),Fo(\lambda x.snore(x))$}
 }
} 
& \\
& 
\dstree{1}{3.5}{
\br[W]{$Ty(t),Fo(sleep(mary))$}{
 \lf{$Ty(e),Fo(mary)$}
 \lf{$Ty(\langle e,t\rangle),Fo(\lambda x.sleep(x))$}
 }
}
\nccurve[ncurv=.6,angleA=270,angleB=160]{->}{M}{W}
\\
\end{tabular}
}\\
\end{tabular}
\caption{DS analysis of relative clause as {\sc Link}ed semantic trees.}\label{fig:link}
\end{figure}

==> intro1.tex <==
With recognition of the dependency of natural language understanding  on context now being thoroughly established (\cite{Heim82,Kamp81,Kamp.Reyle93} and many many others since),  there is 
increasing recognition that to achieve any level of explanatory adequacy, formal models of how interlocutors build on such content across   the dynamic of conversational exchange poses  the next important challenge for grammar developers \cite{Kempson.etal01,Gregoromichelaki.etal11,GinzburgCooper04,Ginzburg12}, since building up of structure and content can take place across several switches of speaker and hearer roles, with context, structure and content, all evolving step by step.  There is also  independently the challenge of what the concept of word meaning amounts to, with both procedural and content-relative aspects to be expressed  \cite{Blakemore87,Potts07}.  What is less often given sufficient emphasis (though see \cite{Cooper12Type}) is that no matter what level of granularity is defined in the modelling of context,  the conceptual content associated with words may nevertheless remain nondeterminate, even fluctuating within the course of a single conversational exchange, often, but not invariably giving rise to requests for clarification, or suggested corrections.  Illustrative of this quasi-independence of content from the specifics of the indexically identified context, is an exchange such as (\ref{ex:burn}), in which the concept of burn is invoked three times over, each with rather different construal.

\enumsentence{
  A (reporting kitchen accident):   I've had an accident. The kitchen's got rather burned.\\
  B:  Did you burn\\
  A: Myself, no fortunately not. Well, only my hair.
}\label{ex:burn}

In (\ref{ex:burn}) B processes  A's utterance, indirectly requesting clarification by re-using the term \textit{burn} though allowing for a possible shift in its construal;  A  picks up on this in completion of B's question, construing it now  not as an attribute of  the room but as a request about what it means for people to get burned.  This, A being now the interrupting speaker, she formulates in terms of that switch, but  rejects her suggested completion as false; though immediately qualifying this dismissal with \textit{well} signalling some form of   correction, indicating  a further shift  in the construal of  \textit{burn},  with her correction now  triggering the understanding that it was her hair that got burned. This exchange illustrates the extent of the problem.  Not only can individuals extend some partial emergent structure which their conversational partner is constructing (understanding it even though incomplete, and developing it   relative to their own shifting  of that context), but they can impose a shift in the content of the concept in question,  even while talking about some single event.

Such conversational exchanges are problematic for conventional sentence-based grammar formalisms in many ways (see \cite{Gregoromichelaki.etal12}); and only one extant grammar formalism  seeks to model such data   directly: Dynamic Syntax (DS) \cite{Kempson.etal01,Cann.etal05,Kempson.etal16TheoreticalLing}.  Adopting an action-based perspective,  DS  defines language as a set of conditional procedures for action, and explicitly represents the partial structures which these act upon at each step in a hearer's (or speaker's) incremental processing.  However, in defining an appropriate  tree-growth algorithm,  DS has so far adopted symbolic approaches to representing content-labelling expressions, using terms from  the epsilon calculus \cite{Kempson.etal01} or a suitable type theory \cite{Purver.etal10}.  Yet these terms are not able to reflect the non-deterministic content characteristically associated with NL content words, as illustrated here; nor are they  directly compatible with the graded judgements that humans make during processing to assess similarity to (or divergence from) expectation \cite{Clark15surfing}.  In this paper, we address these two problems, by defining an incremental probabilistic vector space semantic model  for DS that is able both to express the non-determinism of the word-labels and yet their compositional effectiveness as established incrementally over conversational exchanges, which may include processes of clarification, correction or other modification. The model is notably parallel to the Predictive Processing model currently under development in cognitive neuroscience \cite{FristonFrith15duet,Clark15surfing}, which provides welcome empirical confirmation. %

